E-BLOW: E-Beam Lithography Overlapping aware Stencil Planning for MCC System

Electron beam lithography (EBL) is a promising maskless solution for the technology beyond 14nm logic node. To overcome its throughput limitation, recently the traditional EBL system is extended into MCC system. %to further improve the throughput. In this paper, we present E-BLOW, a tool to solve the overlapping aware stencil planning (OSP) problems in MCC system. E-BLOW is integrated with several novel speedup techniques, i.e., successive relaxation, dynamic programming and KD-Tree based clustering, to achieve a good performance in terms of runtime and solution quality. Experimental results show that, compared with previous works, E-BLOW demonstrates better performance for both conventional EBL system and MCC system.

==> doc/EBLOW.tex <==


\section{E-BLOW Algorithms}
\label{sec:EBLOW}

To provide better scalability, E-BLOW abandons expensive ILP formulation, and integrates a set of novel approximation/speed-up algorithms.
For 1D-OSP, the successive relaxation algorithm and a dynamic programming based refinement are proposed.
For 2D-OSP, based on Simulated Annealing framework, a novel KD-Tree based clustering is presented.

\input{doc/1D}
\input{doc/2D}



==> doc/app_1d.tex <==

\section{More Discussion on S-Blank Assumption}
\label{sec:app_1d}


\begin{figure} [tb]
  \centering
   \subfigure[]{
    \includegraphics[width=0.28\textwidth]{ordering1}
   }
   \hspace{.1in}
   \subfigure[]{
      \includegraphics[width=0.15\textwidth]{ordering2}
    }
   \subfigure[]{
      \includegraphics[width=0.22\textwidth]{ordering3}
    }
    \hspace{.2em}
    \subfigure[]{
      \includegraphics[width=0.15\textwidth]{ordering4}
    }
   \subfigure[]{
      \includegraphics[width=0.22\textwidth]{ordering5}
    }
  \caption{Greedy based Single Row Ordering.}
  %(a)At first all candidates are sorted by blanking space.~(b)One possible ordering solution where each candidate chooses the right end position.~(c)Another possible ordering solution.
  \label{fig:ordering}
  \vspace{-.2in}
\end{figure}

Under the symmetrical blank assumption, the greedy ordering approach can be illustrated in Fig. \ref{fig:ordering},
where four character candidates $A$, $B$, $C$ and $D$ are to be ordered.
In Fig. \ref{fig:ordering}(a), they are sorted decreasingly by blanking space. 
Then all the candidates are inserted one by one.
%Note that each packing can choose left end or right end.
%In other words, packing one by one doesn't mean to be packed from left to right.
From the second candidate, each insertion has two options: left side or right side of the whole packed candidates.
For example, if $A$ is inserted at the right of $D$, $B$ has two insertion options:
one is at the right side of $A$ (Fig. \ref{fig:ordering}(b)), another is at the left side of $A$ (Fig. \ref{fig:ordering}(d)).
Given different choices of candidate $B$, Fig. \ref{fig:ordering}(b) and Fig. \ref{fig:ordering}(c) give corresponding final solutions.
Since from the second candidate each one has two choices, by this greedy approach $n$ candidates will generate $2^{n-1}$ possible solutions. 
But following theorem shows that under the symmetry blank assumption, all these solutions have the same length.




==> doc/app_ebl.tex <==

\section{Background of EBL System}
\label{sec:app_ebl}

%**************************************************************
%               VSB mode and CP mode
%**************************************************************

Conventional EBL system comprises two writing modes: variable shaped beam (VSB) and character projection (CP).
In VSB mode, the entire layout is decomposed into a set of rectangles,
each being shot into resist by one electron beam.
The printing process of VSB mode is illustrated in Fig. \ref{fig:process} (a).
At first the electrical gun generates an initial beam, which becomes uniform through the shaping aperture.
Then the second aperture finalizes the target shape with a limited maximum size.
Since each pattern needs to be fractured into pieces of rectangles and printed one by one, the VSB mode suffers from serious throughput problem.
%For example, the pattern of ``H'' in Fig. \ref{fig:process} (a) is divided into three rectangles and totally it needs three electronic shot.

\begin{figure}[h]
  \centering
  \subfigure[VSB]{\includegraphics[width=0.24\textwidth]{DAC13_VSB}}
  \hspace{-.1in}
  \subfigure[CP]{\includegraphics[width=0.24\textwidth]{DAC13_CP}}
  \caption{Printing process of conventional EBL system.~(a) VSB mode.~(b) Extended CP mode.}
  \label{fig:process}
  \vspace{-.1in}
\end{figure}


%so even simple lines should be exposed by using line pattern characters.


As an improved technique, CP mode is proposed to release the throughput limitation
%\cite{EBL_SPIE2010_Fujimura}
.
As shown in Fig. \ref{fig:process} (b), in the CP mode the second aperture is replaced by a \textit{stencil}.
Some complex shapes, called \textit{characters}, are prepared on the stencil.
The key idea is that if a pattern is pre-designed on the stencil, it can be printed in one electronic shot, by this way the throughput can be improved significantly.
In addition, CP exposure method has a good CD control stability compared with VSB
%\cite{EBL_SPIE08_Maruyama}.
%so even simple lines should be exposed by using line pattern characters.

However, the area constraint of stencil is the bottleneck. 
For modern design, because of the numerous distinct circuit patterns,  only limited number of patterns can be employed on stencil.
Those patterns not contained by stencil are still required to be written by VSB
%\cite{EBL_SPIE09_Manakli}
.
To improve the throughput, the stencil should be carefully designed/manufactured to contain the most repeated cells or patterns.





==> doc/app_ilp.tex <==
%*********************************************
% *             ILP Formulation
% *********************************************

\vspace{-.1in}
\section{ILP Formulation for OSP}
\label{sec:app_ilp}

In this section we will show that besides 1D-OSP, 2D-OSP can be also formulated as integer linear programming (ILP).
At last, as an additional experimental results, we will compare the performances between E-BLOW and the ILP formulations.

% Table of ILP vs. EBLOW
%{{{
\begin{table*}[htb]
\centering
\caption{ILP v.s. EBLOW}
\label{table:small}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
  \hline \hline
  & char & row 	&\multicolumn{3}{c|}{ILP}	& \multicolumn{3}{c|}{E-BLOW}\\
  \cline{4-9}   & \# & len	& shot \#	& char \#	& CPU(s)	& shot \#	& char \#	& CPU(s)\\
	\hline
	1T-1    &6  & 60        &189  &3  &2.0          &213   &3  &0.0     \\
	1T-2    &30 & 60        &1988 &3  &48.9         &2010  &3  &0.0     \\
	1T-3    &15 & 110		&255  &12 &$>$1500      &307   &12 &0.1     \\
	1T-4    &20 & 110		&519  &13 &$>$1500      &519   &13 &0.72    \\
	\hline
	2T-1    &7  & 100		&208  &4  &810          &240   &4  &1.1     \\
	2T-2    &8  & 100		&274  &4  &1381         &305   &4  &1.2     \\
	2T-3    &10 & 100		&360  &5  &$>$1500      &421   &4  &1.5     \\
	\hline
	Total	&- 	&-          &3793 &44   &-		    &4015  &43 &4.62    \\
	Ratio	&- 	&-	        &0.94 &1.02	&-		    &1	   &1  &1       \\
	\hline \hline
\end{tabular}
\end{table*}
%}}}


\vspace{-.05in}
\subsection{2D-OSP ILP Formulation}

%******* ILP notations
%{{{
\begin{table}[htb]
 %\renewcommand{\arraystretch}{1}
 \centering 
 \vspace{-.1in}
 \caption{Notations used in 2D-ILP Formulation}
 \label{table:notations1}
 \begin{tabular}{|l|l|}
 \hline
 \hline
 $W (H)$                  & width (height) constraint of stencil \\
 \hline
 $w_i (h_i)$              & width (height) of candidate $c_i$ \\
 %\hline
 %{\color{blue}  $sl_i (sr_i)$}            & left (right) blanking width of $c_i$
 %\\ 
 %\hline
 %$st_i (sb_i)$            & top (bottom) blanking width of $c_i$\\ 
 \hline
 $o_{ij}^h (o_{ij}^v)$    & horizontal (vertical) overlap between $c_i$ and $c_j$ \\
 \hline
 $w_{ij} (h_{ij})$        & $w_{ij} = w_i - o_{ij}^h$, $h_{ij} = h_i - o_{ij}^v$\\
 \hline
 $p_{ij}$                 & 0-1 variable, $p_{ij} = 0$ if $c_i$ is left of $c_j$ $p_{ij} = 0$\\
 \hline
 $q_{ij}$                 & 0-1 variable, $q_{ij} = 1$ if $c_i$ is below $c_j$\\
 \hline
 $a_i$                    & 0-1 variable, $a_i = 1$ if $c_i$ is on stencil\\
\hline
\hline
\end{tabular}
\vspace{-.1in}
\end{table}
%}}}

Compared with 1D-OSP, 2D-OSP is more general: the blanking spaces of characters are non-uniform along both horizontal and vertical directions. 
The 2D-OSP problem can be also formulated as an ILP formulation (\ref{eq:2ilp}).
For connivence, Table \ref{table:notations1} lists some notations used in the ILP formulation.
The formulation is motivated by \cite{FLOOR_TCAD91_Sutanthavibul}, but the difference is that our formulation can optimize both placement constraints and character selection, simultaneously.
\begin{figure}[htb]
\vspace{-.2in}
\begin{align}
  \textrm{min} \ & T_{total}  				\label{eq:2ilp}\\
  \textrm{s.t. }\  & T_{total} \ge T_{c}^{VSB} - \sum_{i=1}^{n} R_{ic} \cdot a_i, \quad \forall c \in P  \label{2ilp_a}\tag{$5a$}\\
                   &   x_i + w_{ij} \le x_j + W (2+p_{ij}+q_{ij}-a_i-a_j)	\label{2ilp_b}\tag{$5b$}\\
                   &   x_i - w_{ji} \ge x_j - W (3+p_{ij}-q_{ij}-a_i-a_j)	\label{2ilp_c}\tag{$5c$}\\
                   &   y_i + h_{ij} \le y_j + H (3-p_{ij}+q_{ij}-a_i-a_j)	\label{2ilp_d}\tag{$5d$}\\
                   &   y_i - h_{ji} \ge y_j - H (4-p_{ij}-q_{ij}-a_i-a_j)	\label{2ilp_e}\tag{$5e$}\\
                   &   x_i + w_i \le W, \ \  y_i + h_i \le Y				\label{2ilp_f}\tag{$5f$}\\
                   &   p_{ij}, q_{ij}, a_i: \textrm{0-1 variable}			\label{2ilp_g}\tag{$5g$}
\end{align}
\vspace{-.2in}
\end{figure}
where $a_i$ indicates whether candidate $c_i$ is on the stencil, 
$p_{ij}$ and $q_{ij}$ represent the location relationships between $c_i$ and $c_j$. 
We can see that if $a_i = 0$, constraints (\ref{2ilp_b}) - (\ref{2ilp_e}) are not active.
Besides, it is easy to see that when $a_i = a_j = 1$, for each of the four possible choices of $(p_{ij}, q_{ij}) = (0,0), (0,1), (1,0), (1,1)$, only one of the four inequalities (\ref{2ilp_b}) - (\ref{2ilp_e}) are active.
The number of variables is $O(N^2)$, where $N$ is number of characters.

Program (\ref{eq:2ilp}) can be relaxed to linear programming (LP) by replacing constraint (\ref{2ilp_g}) as:
\begin{displaymath}
0 \le p_{ij}, q_{ij}, a_i \le 1
\end{displaymath}
However, similar to the discussion in 1D-OSP, the relaxed LP solution provides no information or guideline to the packing, i.e., every $a_i$ is set as $1$, and every $p_{ij}$ is set as $0.5$.
In other words, this LP relaxation provides no useful information to guide future rounding:
all the character candidates are selected and no ordering relationship is determined.
Therefore we can see that LP rounding method cannot be effectively applied to program (\ref{eq:2ilp}).
%Similar to Lemma \ref{lem:on}, we let $v(ILP_{\ref{eq:2ilp}})$ be the optimal value of the program (\ref{eq:2ilp}), and $v(LP_{\ref{eq:2ilp}})$ be the optimal value of the LP relaxation. We can achieve the following Lemma.

%For brevity we omit the proof here, but we can see that the proof processing is similar to that in Lemma \ref{lem:on}.
%Because of this, E-BLOW adopts a simulated annealing based approximation framework.
%Different from the framework in \cite{EBL_TCAD2012_Yuan}, a novel KD-Tree based clustering is proposed to reduce the problem size.
%As discussed above, 2D-OSP problem comprises several special properties, which make the clustering methodologies quite effective.
%Note that our clustering approaches can not only utilized to reduce the problem size in simulated annealing, but also for the ILP formulation (\ref{2d}).



\vspace{-.05in}
\subsection{ILP vs. E-BLOW}

So far we have formulate both 1D-OSP and 2D-OSP with ILP.
Theoritically ILP can find optimal solution for both problems.
Here we compare ILP results with E-BLOW.
We randomly generate seven benchmarks, four for 1D-OSP (``1T-x") and three for 2D-OSP (``2D-x").
The sizes of all the character candidates are set as $40\mu m \times 40 \mu m$.
The colums ``char \#" and ``row len" list the number of candidates and length of stencil, respectively.
For 1D-OSP benchmarks, the row number is set as $\lfloor \textrm{row len} / 40\rfloor + 2$.
For example, row length $60$ means the row number is $\lfloor 60 / 40 \rfloor + 2 = 3$.
For each mode, we record ``shot \#", ``char \#" and ``CPU(s)",
where ``shot \#" is final number of shots and ``char \#" is number of characters on final stencil, ``CPU(s)" reports the runtime.
From the Table \ref{table:small} we can see that compared with approximation mode, the optimal mode can save $6\%$ of shot number.
However, when the number of candidates is more than $20$ and the row length is more than $100$, the runtime of ILP is unacceptable.


The number of variables in ILP formulations (\ref{eq:1ilp}) and (\ref{eq:2ilp}) are $O(N^2)$.
Since in MCC system $N$ may be as large as $5000$, the number of variables will be around $10^7$.
Although the ILP based algorithm can provide optimal solution, it is impossible to handle such large problem size.
Note that our clustering can be applied not only for ILP mode, but also for the simulated annealing framework.




==> doc/app_proof.tex <==

\vspace{-.1in}
\section{Proof of Theorems}
\label{sec:app_proof}

% ///
%\vspace{-.1in}
\noindent \underline{Proof of Theorem \ref{them:symm}}:

\begin{proof}
It can be proved by recursion. For $p$ candidates, each one with blank space $s_i$. 
Without loss of generality we set $s_1 \ge s_2 \ge \dots \ge s_p$.
Then we try to proof the maximum overlapping space is $f(p) = \sum_{i=2}^p s_i$.
If $p=2$ the theorem is trivial and $f(2) = s_2$.
We assume that when $p=n-1$, the maximum overlapping space $f(n-1) = \sum_{i=2}^{n-1} s_i$.

When $p=n$, since the last candidate can only be inserted at either the left end or the right end, and for any $i<n$, $s_i \ge s_n$, we can find the incremental overlapping space is $s_n$.
Then $f(n) = f(n-1) + s_n = \sum_{i=2}^n s_i$.
\end{proof}



\iffalse
%///
\underline{Proof of Lemma \ref{lem:on}}:
\begin{proof}
Let us first consider a special case where each $profit_i = C$.
Since the objective is trying to maximize the function of $a_{i1}$, the optimal solution of LP would be like this:
for each $i$, $\sum_j a_{ij}=1$ and all the $p_{ij}$ are assigned $0.5$.
By this way the objective function is maximized and all the constraints are satisfied.
We denote $min_s$ as the minimum horizontal slack length of all character, i.e. $min_s = \textrm{min}\{sl_i, sr_i | i = 1, 2, \cdots, n\}$.
Let $p$ be the final character number solved by $(\ref{eq:1ilp})$, and $p'$ be the final number if all character setting slack as $max_s$.
Then $p \le p'$, and given stencil size, $p'$ is a constant.
We can get $v(LP)/v(ILP) = (C \cdot n) / (C \cdot p) = n / p \ge n / p'$, which is proportional to $n$.

For the general case, i.e. for different candidate $i$ and $j$, their profits might be different.
We denote $\alpha = \textrm{max}\{profit_i\}$ / $\textrm{min} \{profit_j\}$,
then $v(LP) / v(ILP) \ge n/(p \cdot \alpha) \ge n/(p' \cdot \alpha)$, which is also proportional to $n$.
\end{proof}
\fi



% ///
%\vspace{-.1in}
\noindent \underline{Proof of Theorem \ref{them:3}}:

\begin{proof}
Let $v(ILP_{3'})$ be the optimal value of the program (\ref{knapsack}), and $v(LPR_{3'})$ be the corresponding LP rounding result described in \cite{Knapsack_JCO00Dawande}.
According to Lemma \ref{lem:2}, $v(LPR_{3'}) \ge 0.5 \cdot v(ILP_{3'})$.
Besides, we denote $v(LPR_{3})$ as the LP rounding result of program (\ref{fast}).
Then using the same rounding method in Lemma \ref{lem:2}, $v(LPR_{3}) \ge 1/\alpha \cdot v(LPR_{3'}) \ge 0.5/\alpha \cdot v(ILP_{3'})$.
\end{proof}




==> doc/bak/bio.tex <==

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/beiyu}}]{Bei Yu}
(S'11) received the M.S. degree in computer science from Tsinghua University, Beijing, China, in 2010.
He is currently pursuing the Ph.D. degree with the Department of Electrical and Computer Engineering, the University of Texas at Austin.
His main research interests include design for manufacturability with emerging nanolithography, and optimization algorithms with applications in VLSI CAD.

%He was with Mentor Graphics, San Jose, CA, in 2011 as an Intern.
He received the Best Paper Award at ASPDAC 2012 and the William J. McCalla Best Paper Award Nomination at ICCAD 2011.
\end{IEEEbiography}

\begin{IEEEbiography}{Kun Yuan}
received the B.S. degree in electronic engineering information science from the University of Science and Technology of China, Hefei, China, in 2004,
and the Ph.D. degree in electrical and computer engineering from the University of Texas, Austin, in 2010.

He was with TeraRoute, Austin, TX, in 2007 and with NVIDIA, Santa Clara, CA, in 2009.
He is currently a Senior Member of Technical Staff with Cadence Design Systems, San Jose, CA.
His current research interests include physical design automation for manufacturability and numerical optimization.

Dr. Yuan received the ISPD Routing Contest Award in 2007, and three Best Paper Awards
(ASPDAC 2010, ISPD 2011, and the IBM Research 2010 Pat Goldberg Memorial Best Paper Award in CS/EE/Math).
\end{IEEEbiography}

\begin{IEEEbiography}{David Z. Pan}
(S'97--M'00--SM'06) received the B.S. degree from Peking University, Beijing, China,
and the M.S. and Ph.D. degrees from the University of California, Los Angeles (UCLA).

From 2000 to 2003, he was a Research Staff Member with the IBM T. J. Watson Research Center, Yorktown Heights, NY.
He is currently an Associate Professor with the Department of Electrical and Computer Engineering, University of Texas, Austin.
He has published over 160 papers in international conferences and journals, and holds eight U.S. patents.
His current research interests include nanometer physical design, design for manufacturability and reliability, vertical integration design and
technology, and design/computer-aided design (CAD) for emerging technologies.

Dr. Pan has served as an Associate Editor for the IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems,
the IEEE Transactions on Very Large Scale Integration Systems,
the IEEE Transactions on Circuits and Systems Part I and Part II,
the Journal of Computer Science and Technology, and the IEEE Circuits and Systems Society Newsletter.
He has served as the Chair of the IEEE CANDE Committee and the ACM/SIGDA Physical Design Technical Committee.
He is in the Design Technology Working Group of the International Technology Roadmap for Semiconductor.
He has served in the technical program committees of major VLSI/CAD conferences, including
ASPDAC (Subcommittee Chair), DAC (Subcommittee Chair), DATE, ICCAD(Subcommittee Chair), ISPD (Program Chair), ISQED (Topic Chair),
ISCAS(CAD Track Chair), SLIP (Publication Chair), GLSVLSI, ACISC (Program Co-Chair), ICICDT (Award Chair), and VLSI-DAT (EDA Track Chair).
He was the General Chair of ISPD 2008, the General Chair of ACISC 2009, and the Steering Committee Chair of ISPD 2009.
He received a number of awards for his research contributions and professional services, including the ACM/SIGDA Outstanding New Faculty Award in 2005,
the NSF CAREER Award in 2007, the SRC Inventor Recognition Award thrice in 2000 and 2008, the IBM Faculty Award four times in 2004--2006, 2010,
the UCLA Engineering Distinguished Young Alumnus Award in 2009, seven Best Paper Awards (SRC Techcon 1998 and 2007, DATE 2009, ICICDT 2009, ASPDAC
2010, ISPD 2011, and the IBM Research 2010 Pat Goldberg Memorial Best Paper Award in CS/EE/Math)
and many other Best Paper Award nominations from DAC/ICCAD/ASPDAC/ISPD, ISPD Routing Contest Awards in 2007, the eASIC Placement Contest Grand Prize in 2009, the IBM Research Bravo Award in 2003, the Dimitris Chorafas Foundation Research Award in 2000,
and the ACM Recognition of Service Award in 2007 and 2008.
He was an IEEE CAS Society Distinguished Lecturer from 2008 to 2009.
\end{IEEEbiography}



==> doc/bak/post.tex <==
% *********************************************************
% *        Post Optimization for Thermal Reduction
% *********************************************************
\section{Post Thermal Optimization}
\label{sec:post}

In this section, given packing result, we show that we can further reduce the thermal consumption using post-optimization method.
For both 1D and 2D cases, the thermal optimization can work under the dynamic programming framework.

%      1D Case
\subsection{1D Thermal Optimization}

Divide and Conquer (or Dynamic Programming) based packing method to reduce thermal consumption.

\subsubsection{1D Solution Propagation}

We start from the first character and set its position to each of two possible choices, i.e. the front and the back of packed row.
This introduces two partial solutions.
For each partial solution, we process the second cell and set its position to each of two choices.
In this way, the algorithm proceeds in a dynamic programming fashion, i.e. it processes each cell in turn according to the topological order.

\subsubsection{1D Solution Pruning}

Without any solution pruning, there are certainly $2^n$ solutions for optimizing $n$ cells.
Therefore, during the solution propaggation process, inferior solutions are pruned for acceleration.

For any two solutions $S_1, S_2$ with the same set of processed cells, $S_2$ is inferior to $S_1$ if ... $>.<!$


%      2D Case
\subsection{2D Thermal Optimization}

\cite{FLOOR_TC91_CKCheng} shows that for tradional floorplanning design, cell flipping problem is NP-Complete.
In physical design, this problem is well studied \cite{FLOOR_ICCAD05_Hao}\cite{FLOOR_DAC06_Sham}.
The problem was shown to be equivalent to finding a minimum cut of a graph with some arcs of negative capacities.

However, the case here is more complicated:
for cell flipping, each cell has only one operation;
here each clusted cell has several possible flipping operation.

We propose a Dynamic Programming framework to solve the problem.

\subsubsection{2D Solution Propagation}

\subsubsection{2D Solution Pruning}


==> doc/bak/prev.tex <==
%============================================
%                           Previous Works
%============================================
\section{Previous Works}
\label{sec:previous}

Many researches have been working on design optimizations for both VSB and CP \cite{EBL_SPIE03_Babin}\cite{EBL_SPIE07_Sugihara}.
When overlappings among characters are not considered, the stencil planning is a character selection problem,
which selects the optimal set of candidates which are placed on a CP aperture mask so the total number of e-beam shots is minimized. 
\cite{EBL_IEICE06_Sugihara}
\cite{EBL_SPIE06_Sugihara} proposed Integer Linear Programming (ILP) based methodologies to select group of characters for minimizing total projection time of both CP and VSB.

Recently, Yuan et al. in \cite{EBL_ISPD2011_Yuan} investigated on new problem of Overlapped aware EBL Stencil Planning (OSP) problems.
They defined two sub problems: 1D-OSP and 2D-OSP, and two frameworks were proposed to handle these two problems, respectively.
In 1D-OSP, an four-phase iterative refinement was processed to conduct one-dimensional stencil design optimization.
A Hamilton-path based approach was developed to solve single-row ordering.
However, the overall framework was based on heuristic framework, so the solution was lack of global optimum.
In 2D-OSP, the problem was transformed into a floorplanning problem, and Sequential Pair (SP) \cite{FLOOR_TCAD96_SP} representation was used in simulated annealing framework.
However, their framework suffers from long runtime penalty.

% *** VSB Design Optimization
%For traditional VSB design, \cite{EBL_SPIE03_Babin}\cite{EBL_SPIE03_Babin2} addressed the sub-field scheduling problem.
%Kahng et al. in~\cite{EBL_SPIE04_Kahng}\cite{EBL_SPIE06_Kahng} addressed the fracturing problem, which partitions a polygon into several basic shapes. 
%An Integer Linear Programming (ILP) based approach and some speeding up heuristics were used to solve the problem. 
%
% *** CP Design Optimization
%For emerging CP design, Sugihara et al. in \cite{EBL_SPIE07_Sugihara} proposed a technology mapping technique for enhancing the throughput of the equipment which adopts both the CP and the VSB methods. 
%%The proposed technology mapping technique reduces the number of EB shots to draw an entire chip.
%In~\cite{EBL_SPIE04_Yasuda} Yasuda et al. proposed a multi-column-cell (MCC) system, which can project multiple characters in parallel to achieve the higher throughput than sequential projection systems.
%\cite{EBL_SPIE09_Sugihara}\cite{EBL_ISCAS06_Sugihara} proposed a character size optimization technique to enhance throughput of MCC lithographic systems. 
%The optimization problem was formulated as a Mixed Integer Nonlinear Programming (MINLP), and a heuristic method was adopted to linearize the problem.



==> style.tex <==

\renewcommand{\algorithmicrequire}{\textbf{Input:}}  % Use Input in the format of Algorithm
\renewcommand{\algorithmicensure}{\textbf{Output:}} % Use Output in the format of Algorithm


%theorem
\theoremstyle{plain}
\theoremheaderfont{\normalfont\bfseries}\theorembodyfont{\slshape}
\theoremsymbol{\ensuremath{\diamondsuit}} \theoremseparator{:}
\newtheorem{mytheorem}{Theorem}


% problem
\theoremstyle{plain}
\theoremsymbol{\ensuremath{\clubsuit}}
\theoremseparator{.}
\newtheorem{problem}{Problem}


%lemma
%\theoremstyle{changebreak}
\theoremsymbol{\ensuremath{\heartsuit}}
%\theoremindent0.5cm
%\theoremnumbering{greek}
\newtheorem{mylemma}{Lemma}

%example
\theoremstyle{change}
\theorembodyfont{\upshape}
\theoremsymbol{\ensuremath{\ast}}
\theoremseparator{}
\newtheorem{myxample}{Example}

%proof
\theoremheaderfont{\sc}\theorembodyfont{\upshape}
\theoremstyle{nonumberplain} \theoremseparator{}
\theoremsymbol{\rule{1ex}{1ex}}
\newtheorem{myproof}{Proof}

%definition
\theoremstyle{plain} \theoremsymbol{\ensuremath{\clubsuit}}
\theoremseparator{.}
\newtheorem{mydefinition}{Definition}


%%%%%%%%%%%%%%%%%%%%%%%%%%%% Setting to control figure placement
% These determine the rules used to place floating objects like figures
% They are only guides, but read the manual to see the effect of each.
%\renewcommand{\topfraction}{1.9}
%\renewcommand{\bottomfraction}{1.9}
%\renewcommand{\textfraction}{.1}
%


